The impact of ionised outflows from z$\sim$2.5 quasars is not through instantaneous in-situ quenching: the evidence from ALMA and VLT/SINFONI

We present high-resolution ($\sim$2.4\,kpc) ALMA band 7 observations (rest-frame $\lambda \sim 250\mu$m) of three powerful z$\sim$2.5 quasars ($L_{\rm bol}=10^{47.3}$-$10^{47.5}$ ergs s$^{-1}$). These targets have previously been reported as showing evidence for suppressed star formation based on cavities in the narrow H$\alpha$ emission at the location of outflows traced with [O~{\sc iii}] emission. Here we combine the ALMA observations with a re-analysis of the VLT/SINFONI data to map the rest-frame far-infrared emission, H$\alpha$ emission, and [O~{\sc iii}] emission. In all targets we observe high velocity [O~{\sc iii}] gas (i.e., W80$\sim$1000--2000\,km\,s$^{-1}$) across the whole galaxy. We do not identify any H$\alpha$ emission that is free from contamination from AGN-related processes; however, based on SED analyses, we show that the ALMA data contains a significant dust-obscured star formation component in two out of the three systems. This dust emission is found to be extended over $\approx$1.5--5.5\,kpc in the nuclear regions, overlaps with the previously reported H$\alpha$ cavities and is co-spatial with the peak in surface brightness of the [O~{\sc iii}] outflows. In summary, within the resolution and sensitivity limits of the data, we do not see any evidence for a instantaneous shut down of in-situ star formation caused directly by the outflows. However, similar to the conclusions of previous studies and based on our measured star formation rates, we do not rule out that the global host galaxy star formation could be suppressed on longer timescales by the cumulative effect of quasar episodes during the growth of these massive black holes.

==> Tables/Table_phot_vert.tex <==
\resizebox{0.99\paperwidth}{!}{\begin{tabular}{@{}lccc@{}} 
\hline 
\hline 
Band & HB8903 & LBQS01 & 2QZJ00
\hline 

(1) ATLAS u 
(2) ATLAS g
(3) ATLAS r
(4) ATLAS i 
(5) ATLAS z
(6) Pan g
(7) Pan r
(8) Pan i
(9) Pan z
(10) Pan y
(11) 2MASS J
(12) 2MASS H
(13) 2MASS K
(14) Wise W1
(15) Wise W2
(16) Wise W3
(17) Wise W4
(18) ALMA B7
(19) ALMA B3
(20) Radio (1.4 GHz)
 



\hline 
\end{tabular}}

